Traceability Transformed: Generating more Accurate Links with Pre-Trained BERT Models

Software traceability establishes and leverages associations between diverse development artifacts. Researchers have proposed the use of deep learning trace models to link natural language artifacts, such as requirements and issue descriptions, to source code; however, their effectiveness has been restricted by availability of labeled data and efficiency at runtime. In this study, we propose a novel framework called Trace BERT (T-BERT) to generate trace links between source code and natural language artifacts. To address data sparsity, we leverage a three-step training strategy to enable trace models to transfer knowledge from a closely related Software Engineering challenge, which has a rich dataset, to produce trace links with much higher accuracy than has previously been achieved. We then apply the T-BERT framework to recover links between issues and commits in Open Source Projects. We comparatively evaluated accuracy and efficiency of three BERT architectures. Results show that a Single-BERT architecture generated the most accurate links, while a Siamese-BERT architecture produced comparable results with significantly less execution time. Furthermore, by learning and transferring knowledge, all three models in the framework outperform classical IR trace models. On the three evaluated real-word OSS projects, the best T-BERT stably outperformed the VSM model with average improvements of 60.31% measured using Mean Average Precision (MAP). RNN severely underperformed on these projects due to insufficient training data, while T-BERT overcame this problem by using pretrained language models and transfer learning.

==> introductionCOPYORIGINAL.tex <==
During the development of software projects, developers will produce various artifacts along with the source code to systematically control the quality and progress. Artifacts such as requirement, design definition, and test case are all written in natural language and evolving as the project proceeding. The technique of mining and recovering relationships among software artifacts and therefore to trace the life cycles of software artifacts is known as software traceability. The importance of traceability in software projects has been widely recognized by the project stakeholders. With the help of software traceability, stakeholders can effectively conduct a diverse set of engineering activities such as impact analysis, compliance validation, and even bug locating \cite{}. Despite the great value of traceability, the procedures of manual trace link generation are arduous and error-prone \cite{}. It is therefore challenging to directly apply traceability in production. 

Researchers therefore propose various automated approaches to reduce the manual efforts for trace link generation and maintenance\cite{}.
%Javed et al. conduct a survey on software tractability, and categorized traceability approaches into six categories \cite{javed2014systematic} based on their underlying techniques. Among all these approaches, the Information Retrieval (IR) based and Machine Learning (ML) based methods are mostly discussed and investigated by researches. 
For example, trace models built upon Vector Space Model (VSM), Latent Semantic Indexing (LSI), and Latent Dirichlet Allocation (LDA) have been widely adopted for recovering the relationships from high level software requirements to concrete design definitions\cite{}. And Rath et al. \cite{rath2018traceability} leveraged Decision Tree (DT) and Support Vector Machine (SVM) to learn the temporal dependencies between git issues and commits, and recovered the missing links between these two kinds of artifacts. 

To achieve trusted traceability, several researchers have propose to integrate deep learning (DL) techniques to recover the missing links underlying software artifacts \cite{borg2017traceability, zhao2017using}.
Although DL trace models have aroused attention from traceability community, few studies have been conducted to explore deep learning based trace model. Since 2017, only Guo et al. \cite{} proposed a Recurrent Neural Network (RNN) based architecture to address the tracing challenging in safety-critical software projects. In that study, researchers evaluated two types of RNN trace models (LSTM and GRU) by applying them to recover links between subsystem requirements and design definitions. 
We believe there are two main factors obstructing the adoption of deep learning techniques in software traceability studies. The first one is the sparsity of training data. 
Although, deep learning based techniques tend to provide results with higher quality, it requires a large volume of training data. Manually created trace links in software projects are usually not sufficient for supporting the training steps of deep learning techniques. 
Scalability is the other obstruction. Since deep learning techniques incorporate multi-layer neural networks, deep neural networks is significantly slower than other methods. For trace tasks with large volume of candidate links, a deep learning based trace model can be easily overwhelmed.
%may not be able to produce trace results in time. 

In this study, we explore deep learning based trace solutions which are capable of addressing the above two constraints at the same time. We propose a Language Model (LM) based traceability model that are 1) able to provide trustworthy trace links, 2) applicable on projects with limited training data, and 3) scalable to large projects with low time complexity. Our approach leverages BERT (\textbf{B}idirectional \textbf{E}ncoder \textbf{R}epresentations from \textbf{T}ransformers) as its underlying language models, thus we name it as Trace BERT (T-BERT) for the convenience of reference. T-BERT refers to a group of BERT-based architectures applicable for traceability tasks, including single BERT, twin BERT and siamese BERT architecture. We compare the effectiveness of those three types of architectures by applying them to address the tracing challenge between Natural Language Artifacts (NLAs) and Programming Language Artifacts (PLAs). For clarification, we refer NLAs as the artifacts whose main language is natural language, e.g. feature request, bug reports, improvements, requirements, and design definition. And we refer PLAs as artfaicts whose main language is programming language, e.g. code files, code snippets, function definitions and code change sets. Actually, we approach is robust to NL-PL intermingle artifacts, because PLA such as source code will usually contains comments in natural language, and NLA such as bug reports may refer code snippets in natural language as well. To be more specific, our study focus on tracing from issue discussions to code change sets within commits for open source projects on Github. 

In the remaining of this paper, \todo{we firstly balal in Section I. Then we balala Section II.} 






%To address the data sparsity issue, researchers proposed pre-trained deep learning models as solutions. This approach divide the training stage into pre-training and fine-tuning phases. In pre-training phase, deep learning models are constructed with enormous and highly available dataset with unsupervised or semi-supervised training tasks. And then in fine-tuning phase, researchers will optimize the models on problem-related yet small datasets to specialize the dataset to target problem, which is also known as downstream problems. The idea behind this type of approaches is that knowledge learned from pre-training tasks on general and large dataset can be effectively transferred to downstream tasks suffering from data sparsity. 





% discuss the weankness of deep learning approaches on traceability

%Compare with IR based methods, such as Vector Space Model (VSM), Latent Semantic Indexing (LSI), and Latent Direchlet Allocation (LDA), ML based trace model tend to generate trace link with higher quality \cite{}. Because machine learning models such as neural networks are more versatile than IR models to learn the complex patterns hidden in dataset. Multiple studies have illustrated the great effectiveness of adopting deep learning techniques for addressing traceability challenges. However, these methods all requires a large volume of training data with manually created labels to supervise the model training. Unfortunately,  train datasets at such a scale are rarely available, manually labeled trace links can be either missing, incomplete or inaccurate in real-world projects. Meanwhile, deep learning based methods can be computationally expensive in general, this issue occurs not only at model training phase but also at the model applying phase regarding the dense layers in deep learning models. For above two reasons, deep learning based approach are less applicable than IR based models which are lightweight and require no supervision.

% Actually, both of the dataset sparsity and speed issues are ubiquitous in general Natural Language Processing (NLP) domains. To address the dataset issue, researchers proposed pre-trained deep learning models as solutions. This approach divide the training stage into pre-training and fine-tuning phases. 
% In pre-training phase, deep learning models are constructed with enormous and highly available dataset with unsupervised or semi-supervised training tasks. And then in fine-tuning phase, researchers will optimize the models on problem-related yet small datasets to specialize the dataset to target problem, which is also known as downstream problems. 
% The idea behind this type of approaches is that knowledge learned from pre-training task on general and large dataset can be effectively transferred to downstream tasks suffering from data sparsity. The pre-trained models usually provide better starting points for model optimization than the randomly seeded ones, and therefore to reduce the likely-hood of trapping models in local optimality to improve the overall performance. Benefit from the small size of datasets, fine-tuning a pre-trained model take significant less time than training a regular deep learning model. Although, pre-training such models are incredibly expensive, the pre-training phase only need to be done once and can be reused for various downstream tasks.
% Another approach to addressing the speed issue is a transformer based deep learning model. Ashish  et al. firstly proposed attention mechanism in their study to address the machine translation challenge \cite{vaswani2017attention}. The attention enhanced neural layers, illustrated in Fig.~\ref{}, are known as Transformer layers. Sequentially, the models constituted by this type of layers are named as Transformers. The transformer based neural machine translation model not only outperforms the Google Neural Machine Translation model in accuracy but also required less time on training. This is accomplished through a mechanism known as multi-head attention, which allow transformers to focus on different positions in a sentence in a parallel manner.

% \textbf{B}idirectional \textbf{E}ncoder \textbf{R}epresentations  from \textbf{T}ransformers (BERT), proposed by Devlin et al. , is a combination of pre-trained model and transform for addressing general purpose NLP tasks \cite{devlin2018bert}. BERT is pretrain as a general Language Model (e.g. for English) and then specialized for dedicated task. Various studies have show that BERT and its variants are capable of handling a rich set of NLP challenging, including question answering, document classification, machine translation, sentimental recognition and text generation \cite{}.However, no study has been conducted to apply BERT or other transformer based methods upon software traceability. Most recent works deep learning-based traceability approaches are build upon Recurrent Neural Network (RNN) \cite{}. Regarding the fact that BERT based methods are continuously creating new state-of-the-art in other NLP domains which were dominated by RNN, it is reasonable to hypothesis that transformers are better fits than RNN for addressing software traceability problem as well. 
% Therefore, in this study, we propose a dual BERT architecture for addressing the link generation challenge among source code and other NL artifacts such as requirement, design definition and test case. For the convince of reference, we name it as T-BERT (Traceability BERT)

% Gururangan et al. claim in their study of domain-adaptive pretraining (DAPT) that, continued pertaining on related domain corpus can consistently improves performance on the downstream tasks in that domain disregarding the size of training corpus \cite{}. We therefore adopt a three-fold training procedure including pretrain, post-pretrain and fine-tune. In pretrain step, we construct regular language models with standard pertaining techniques. Then in post-pretrain, we specialize the the LM with a retriving tasks between source code and code comments. Finally, in fine-tune step, we train the model with project artifacts and supervise it with human labeled links. In our post-pretrain and fine-tune steps, we combine the online negative example sampling techniques to improve the model performance which alleviated the glass ceiling problem observed by Jin et al. \cite{} in their study. Our result show that \todo{*update with definitive results*}.



==> tables/tab_hyperparam.tex <==
\begin{table}[ht]
	\centering
    \caption{Hyper-parameter for T-BERT models in post-pretraining and fine-tuning}
    
    \begin{tabular}{|p{3cm}|p{5cm}|}
    \hline
    Epoch & 8 - post-pretrain \\
    & 400 - fine-tune \\ \hline
    Batch Size & 8 \\ \hline
    Batch Accumulation Step & 8 \\ \hline
    Dropout rate & 0.2 \\ \hline
    Init Learning Rate (lr) & 1.00E-05 \\ \hline
    LR scheduler & linear \\ \hline
    Warm-up Step & 0 \\ \hline
    Hidden State Dim & 512 \\ \hline
    Max Seq Length & 512 \\ \hline
    Adam Epsilon & 5.00E-05 \\ \hline
    Gradient Clip Value & 1 \\ \hline
    \end{tabular}
	\label{tb_tab:hyper_param}
	\vspace{-12pt}
\end{table}
